Item-side Fairness of Large Language Model-based Recommendation System

Recommendation systems for Web content distribution intricately connect to the information access and exposure opportunities for vulnerable populations. The emergence of Large Language Models-based Recommendation System (LRS) may introduce additional societal challenges to recommendation systems due to the inherent biases in Large Language Models (LLMs). From the perspective of item-side fairness, there remains a lack of comprehensive investigation into the item-side fairness of LRS given the unique characteristics of LRS compared to conventional recommendation systems. To bridge this gap, this study examines the property of LRS with respect to item-side fairness and reveals the influencing factors of both historical users' interactions and inherent semantic biases of LLMs, shedding light on the need to extend conventional item-side fairness methods for LRS. Towards this goal, we develop a concise and effective framework called IFairLRS to enhance the item-side fairness of an LRS. IFairLRS covers the main stages of building an LRS with specifically adapted strategies to calibrate the recommendations of LRS. We utilize IFairLRS to fine-tune LLaMA, a representative LLM, on \textit{MovieLens} and \textit{Steam} datasets, and observe significant item-side fairness improvements. The code can be found in https://github.com/JiangM-C/IFairLRS.git.

==> 0001Introduction_previous_backup.tex <==
\section{Introduction}

% 
The Recommendation System (RS) plays an important role in daily life, which mitigates the predicament of information overload.
% 
Recently, with the rise of ChatGPT~\cite{}, more and more researchers have focused on Large Language Models (LLMs) in the field of recommendation and obtained better performance than conventional sequential recommendation models~\cite{tallrec, bigrec}. 
% However, using LLMs for recommendations still faces fairness issues which may lead to problems such as Matthew effect~\cite{} and filter bubble~\cite{}.
Despite the potential advantages offered by LLMs in the recommendation domain, their utilization is not without challenges, particularly pertaining to issues of fairness. 
% These may hurt the enthusiasm of both creators and users.
These challenges encompass the manifestation of Matthew effect~\cite{}, and the filter bubbles~\cite{}, which possess the capacity to dampen the enthusiasm of both creators and users alike.

In this paper, we focus on the item-side fairness issues in LLMs for recommendations, which have received limited attention in prior research efforts.
The item-side fairness discussed in conventional recommendation works requires that the RS should not exhibit bias toward any specific item group.
% The item-side fairness requires that the RS should not exhibit bias toward any specific item group.
%%% x
% In view of inherent biases within datasets, it is observed that highly popular items are more likely to be recommended, thereby hindering the equitable exposure and exploration of less mainstream items.
% Similarly, LLM-based recommendations can potentially exhibit unfairness towards distinct genres of item groups, resulting in users receiving excessive information of the same type.
% To avoid the Matthew effect and the filter bubbles, the RS cannot be biased toward any groups.
For example, previous works~\cite{} have shown that highly popular items are more likely to be recommended in conventional RS, thereby hindering the equitable exposure and exploration of less mainstream items. 
Similarly, if recommendations exhibit unfairness towards distinct genres of item groups, it will result in users receiving excessive information of the same type.
However, regardless of the chosen division or perspective, the underlying essence remains unchanged.
% Previous works~\cite{bigrec} have shown that the LLM for recommendation heavily relies on the semantic information stored in LLM.
Previous studies~\cite{bigrec} have demonstrated that the effectiveness of LLMs for recommendation tasks heavily depends on the utilization of semantic information stored in the LLM framework.
% Therefore, item-side fairness in LLMs for recommendations is crucial in the development of recommendation algorithms.
Therefore, in contrast to conventional approaches, the consideration of item-side fairness of LLMs for RS requires the examination of two distinct scenarios: semantic independence and semantic correlation scenarios.
% By prioritizing fair and unbiased recommendations, the overall experience for both creators and users can be significantly enhanced.
In order to fully explore the item-side fairness of LLMs for RS, it is necessary to analyze the two conditions separately.

% In this work, we first design the experiments on BIGRec~\cite{bigrec} to probe the item-side fairness of LLMs for recommendations and explore the root causes of unfairness issues in the model. 
Within this work, we commence by designing the experiments on BIGRec~\cite{bigrec} to probe the item-side fairness of LLMs for recommendations and explore the root causes of unfairness issues in the model. 
% In our observation, we find that LLM-based recommendations are affected by the popularity of items significantly, which is mitigated by the bi-step grounding paradigm of BIGRec.
To comprehensively examine the various forms of item-side fairness, we adopt two distinct perspectives in our analysis.
In the semantic independence scenario, we employ popularity as the criterion to partition the data into diverse groups.
% To evaluate the item-side fairness in the semantic correlation scenario, we choose genre as the criterion.
In the semantic correlation scenario, we evaluate the item-side fairness of models for different genre groups.
In our observation, we discover that LLM-based recommendations are substantially influenced by the popularity of items, which is alleviated through the bi-step grounding paradigm employed by BIGRec.
% And influenced by semantic information, the LLM-based recommendations are more unfair for different genre groups compared with traditional sequential recommendations.
Furthermore, we find that the LLM-based recommendations exhibit a greater degree of unfairness towards distinct genre groups compared with traditional sequential recommendations.
Meanwhile, because category information and semantics are intertwined, the bi-step grounding will introduce a new problem of fairness for different genres. 

% 介绍我们的新方法
Then, we propose multiple methods both 

% 贡献
In conclusion, our contributions are as follows:
\begin{itemize}[leftmargin=*]

\item We reveal the unfairness issue of the LLM-based Recommendation System and conduct multiple experiments to probe the influence of different parts of BIGRec.

\item We propose multiple methods to mitigate the unfairness of the model, which integrate into the different phases of training.

\item Various experiments are conducted on different datasets to show the effectiveness of our proposed method and we analyze the advantages and disadvantages of these methods.
\end{itemize}

==> 0002Preliminary_backup1107.tex <==
\section{Preliminary}
In this section, we first elaborate on the evaluation of item-side fairness in LLM-based recommendation.
Afterward, we introduce BigRec \cite{bigrec}, one of the most recent LLM-based recommenders, which serves as the backbone model in our method.



%怎么改啊 怎么抽象啊 most recent 行不行 recommender怎么了
\subsection{Evaluation of Item-side Fairness}
\label{sec:2_1}
% 介绍fairness的定义
% Fairness within recommendation systems can be categorized into two dimensions: user-side fairness and item-side fairness.
% % The user-side fairness aims to make fair recommendations to users with different sensitive attributes.
% User-side fairness \cite{fairllm, up5} focuses on ensuring equitable recommendations for users possessing diverse sensitive attributes.
In this work, the goal of item-side fairness is to provide fair recommendations \wrt different groups of items.

Let $\mathcal{H}$ denote the set of interaction sequences in testing data, $\mathcal{P}$ denote the set of top-K recommendation results at the testing phase, and $\mathcal{G}$ denote the set of item groups.  

Given an item $i$ and a group $G \in \mathcal{G}$, we define the identity function:
\begin{equation}
\mathbb{I}(i \in G) = 
\begin{cases}
1, & \text{item $i$ can be devided into group $G$}  \\
0, & \text{otherwise} 
\end{cases}.
\end{equation}

Accordingly, the occurrence probability of a group $G$ in the testing interaction sequence set $\mathcal{H}$ can be formulated as:
\begin{equation}
\label{eq:count}
    \textbf{GH}(G) = \frac{\sum_{H \in \mathcal{H}}\sum_{i \in H} \mathbb{I}(i \in G) }{\sum_{G' \in \mathcal{G}}\sum_{H \in \mathcal{H}}\sum_{i \in H} \mathbb{I}(i \in G')}.
\end{equation}

Similarly, the occurrence probability of a group $G$ in the testing top-K recommendation result set $\mathcal{P}$ can be formulated as:
\begin{equation}
\label{eq:count_predict}
    \textbf{GP}(G) = \frac{\sum_{P \in \mathcal{P}}\sum_{i \in P} \mathbb{I}(i \in G) }{\sum_{G' \in \mathcal{G}}\sum_{P \in \mathcal{P}}\sum_{i \in P} \mathbb{I}(i \in G')}.
\end{equation}

To this end, we can define \textbf{Group Unfairness (GU)} \wrt group $G$ as:
\begin{equation}
    \textbf{GU}(G) = \textbf{GP}(G) - \textbf{GH}(G),
\end{equation}
which evaluates the unfairness of a certain group $G$ at the testing phase: $\textbf{GU}(G) > 0$ suggests that the recommender tends to exceedingly recommend items from group $G$, while $\textbf{GU}(G) < 0$ implies the recommender might overlook group $G$. Both cases could result in item-side unfairness issue.



Following prior studies \cite{Calibrated, Calibrated2}, we evaluate item-side fairness in recommendation by defining the following metrics:


% Likewise, item-side fairness necessitates that recommendation systems provide fair and unbiased recommendations for diverse groups of items. 
% Nevertheless, it is important to note that fair recommendations do not imply that different groups will receive the same level of exposure.
% For instance, consider a scenario where items are divided into groups based on their popularity, and both the highest and lowest popularity groups are given equal exposure. 
% In this case, although it may seem fair in terms of equal treatment, it could result in an unfair outcome for the high-popularity group. 
% % Thus, the aim of item-side fairness is to minimize any unfair advantages or disadvantages among different item groups, rather than enforcing identical exposure for all groups.
% Therefore, the objective of item-side fairness is to minimize the occurrence of inequitable treatment toward disadvantaged groups and preferential treatment toward advantaged individuals, rather than enforcing uniform treatment for all groups.
% The key is to investigate whether RS exhibits prejudice or favoritism toward specific item groups, resulting in unequal exposure for said groups compared to their historical interaction sequence.
% In order to assess the item-side fairness of the RS, we follow the thought of \cite{Calibrated, Calibrated2} and propose several evaluation measures:
% % 定义
% \begin{definition}[Item-side fairness evaluate methods]
% % For several interaction sequences $H$, we can count the number of items of a certain genre $g$ in an interaction sequence $h$, which is expressed as $C(h, g)$. And for the outputs $P$, we also use $C(p, g)$ as the number of items belonging to genre $g$ in the prediction $p$.
% In the case of multiple interaction and prediction sequences denoted as $H$ and $P$, we can quantify the occurrence of items belonging to a specific group $g \in G$ within an interaction sequence $h$ by using the notation $C(h, g)$. Similarly, we employ the notation $C(p, g)$ to represent the count of items categorized under group $g$ within the prediction $p$.


% \textbf{Group Bias (GB)} The bias of a certain group $g$ can be denote as:
% \begin{equation}
%     \label{eq:Group_Bias}
%     GB(g) = \frac{\sum_{p\in{P}}C(p, g)}{\sum_{g^*\in{G}}\sum_{p\in{P}}C(p, g^*)} - \frac{\sum_{h\in{H}}C(h, g)}{\sum_{g^*\in{G}}\sum_{h\in{H}}C(h, g^*)}.
% \end{equation}

% \textbf{Mean Item-side Fairness}
% Note that our objective is to evaluate the fairness of RS; we focus on two aspects of metrics: 

\begin{itemize}[leftmargin=*]
    \item \textbf{Mean Group Unfairness (MGU)} evaluates the overall fairness:
        \begin{equation} \label{eq:MGB}
            \textbf{MGU} = \frac{1}{|\mathcal{G}|}\sum_{G \in \mathcal{G}}|\textbf{GU}(G)|,
        \end{equation}
    \item \textbf{Disparity Group Unfairness (DGU)} measures the disparity between the maximum and minimum Group Unfairness, which could evaluate the upper bound of item-side fairness of recommender:
        \begin{equation} \label{eq:DGB}
            \textbf{DGU} = \underset{G \in \mathcal{G}}{\text{argmax}} \ \textbf{GU}(G) - \underset{G \in \mathcal{G}}{\text{argmin}} \ \textbf{GU}(G).
        \end{equation}
\end{itemize}

% \end{definition}

% Equation~\eqref{eq:Group_Bias} evaluates the bias of the proportion of a specific group in historical interaction sequences and prediction sequences, which denotes the prejudice or favoritism of RS for this group. 
% Equation~\eqref{eq:MGB} quantifies the overall fairness of the RS, where a value closer to 0 indicates a higher level of fairness in the model.
% Finally, Equation~\eqref{eq:DGB} calculates the distance between the highest and the lowest GB, which serves as a measure of both the fairness and stability of the model.

In the experiment, we adopt the all-ranking protocol \cite{dros} to obtain the top-K recommendation results.
Consequently, top-K evaluation can also be employed in the defined fairness metrics, which can be denoted as $\textbf{MGU}@K$ and $\textbf{DGU}@K$. 

% For the Equation~\eqref{eq:MGB} and Equation~\eqref{eq:DGB} we follow the all-ranking protocol \cite{dros} to get the prediction sequences. 
% In this paper, the $k$ of $MGB@k$ and $DGB@k$ denote the top $k$.   

% \subsection{A Bi-Step Grounding Paradigm for Large Language Models in Recommendation Systems}
\subsection{Brief on BIGRec}
\label{sec:bigrec}
Recently, there is emerging work focusing on the application of LLMs in recommendation \cite{bigrec, tallrec, XXX}, from which we can summarize a general pipeline: transferring interaction data in recommendation into natural language and prompting LLMs for recommendation results.
In this paper, we target at investigating item-side fairness in LLM-based recommendation, and select BIGRec \cite{bigrec} as the backbone model in our experiment since XXXX.
Therefore, we present a brief introduction on BIGRec in this section.


Following the general pipeline of applying LLMs in recommendation, BIGRec first transfers interaction data into textual prompts and employs the instruction-tuning approach to fine-tune LLMs and generate descriptions of recommendation results.
However, the generated descriptions are not guaranteed to exist in the actual candidate item set.
To deal with this issue, BIGRec designs a delicate grounding paradigm to precisely locate the actual items for recommendation.
Specifically, let \textbf{oracle} and $\textbf{emb}_i$ denote the token embeddings (\ie latent representations) of the generated descriptions and the description of item $i$ respectively.
BIGRec calculates their L2 distance as:
\begin{equation}
\label{eq:distance}
    D_i = ||\textbf{emb}_i - \textbf{oracle}||_2.
\end{equation}
Thereafter, BIGRec would select the K-nearest items as the recommendation results, based on the L2 distance, to complete the top-K recommendation.





% Our experimental investigation commences with a representative work, BIGRec \cite{bigrec}, which is a bi-step grounding paradigm employed to align the LLMs for RS. 
% BIGRec has several advantages: 1) BIGRec could obtain comparable and even better performance than conventional sequential recommendation methods; 2) BIGRec has a clear structure and we could conveniently explore more details of item-side fairness of LLMs.
% The core of BIGRec lies in its ability to ground the output of LLMs from language space to the actual item space by utilizing a two-step grounding process. 
% % For a special recommendation task, BIGRec first grounds the output of LLMs from the language space to the recommendation space by instruction-tuning. 
% Firstly, BIGRec begins with an instruction-tuning phase on the alpaca self-instruct data \cite{alpaca} using LLaMA \cite{LLaMA}. 
% Then, for a special recommendation task, BIGRec performs instruction-tuning to ground the output of LLMs from the language space to the recommendation space.
% The recommendation space is a sub-space of language space that encompasses a diverse array of entities.
% % These entities can fulfill the user's preferences, but some of them are imaginary items in a particular task, such as ``Iron Man(Sichuan dialect)", which is infeasible in recommendations.
% These entities within the recommendation space could satisfy the user's preferences.
% However, it is important to acknowledge that some of the entities may be imaginary items specific to the task. 
% For instance, an infeasible recommendation would be "Iron Man (Sichuan dialect)", which is not a realistic item for recommendation purposes.

% Therefore, the second step, grounding the output of LLMs from recommendation space to actual item space, is crucial in effectively utilizing LLMs for making recommendations. 
% % The actual item space contains only the actual items in the recommendation space which are special by the recommendation tasks.
% The actual item space exclusively contains the real items that are pertinent to the recommendation task within the recommendation space. 
% BIGRec aligns the output of LLMs with real-world items based on the representations of LLMs to ground the output to actual item space.
% Specifically, BIGRec extracts the latent representation of the generated tokens and the embedding of the actual items.
% Then, BIGRec ranks these actual items by calculating the L2 distance between their embeddings:

% \begin{equation}
% \label{eq:distance}
%     D_i = ||emb_i - oracle||_2,
% \end{equation}

% where $emb_i$ represents the embedding of the i-th item in a certain recommendation task, and $oracle$ denotes the embedding of the outputs generated by the LLM.

% % In this way, BIGRec paradigm can fully exploit the potential of LLMs and attain performance on par even with conventional models, while trained by fewer samples. 
% By employing the BIGRec paradigm, the full potential of LLMs can be harnessed, leading to comparable performance with conventional models, even when trained with fewer samples.
% % However, \cite{bigrec} indicates that LLMs rely heavily on semantics for recommendations, which may result in unfairness of recommendations.
% However, it is important to note that according to \cite{bigrec}, LLMs heavily rely on semantics for generating recommendations, which could potentially introduce biases and unfairness in the recommendation outcomes. 
% In this paper, we undertake a comprehensive investigation into the item-side fairness of the LLM for recommendations within the BIGRec paradigm. 
% Furthermore, we propose measures to enhance the fairness of the LLM and address any potential biases that may arise during the recommendation process.

==> 0003ProbeBACKUP.tex <==
\section{Probe the Item-side Fairness of LLM}
In this section, we conduct experiments to answer the following research questions:

\begin{itemize}[leftmargin=*]
    \item \textbf{RQ1:} How to evaluate the item-side fairness of the model in diverse scenarios?
    \item \textbf{RQ2:} Do LLMs for recommendations have more item-side fairness than conventional methods?
    \item \textbf{RQ3:} What is the difference of fairness between semantic independent scenarios and semantic correlation scenarios?
\end{itemize}

\subsection{Experiment Setting}
\subsubsection{Datasets}
\label{sec:4_1_1}

\begin{table}[htbp]
    \caption{The statistics of the datasets.}
    \label{tab:datasets}
    \begin{tabular}{cccc}
                \hline 
    Datasets     & \#items & \#interactions & \#sequences \\
                \hline
    MovieLens1M & 3,883  & 1,000,209      & 939,809   \\
    Steam       & 14,662 & 7,793,036      & 1,620,946 
                \\\hline    
\end{tabular}  
\end{table}

We conduct experiments on two datasets: MovieLens1M\footnote{https://grouplens.org/datasets/movielens/1m/.} and Steam\footnote{https://jmcauley.ucsd.edu/data/amazon/.}. 
The number of items and the number of interactions are in Table~\ref{tab:datasets}. 
We follow the setting of the BIGRec, to simulate real-world sequential recommendation scenarios, we divided each user's interactions into several sequences based on the timestamp of interactions.
Each sequence consists of ten periods, representing a temporal unit, and is accompanied by a target item for recommendation purposes.
Subsequently, we split the periods of datasets into training, validation, and
testing sets using a ratio of 8:1:1 based on the time.
By ensuring that the predicted interactions during testing occur after all the interactions observed during training, we effectively prevent any leakage of information from the testing phase into the training phase.

To answer the \textbf{RQ1}, we intentionally employ two distinct methodologies for splitting these datasets: 

\begin{itemize}[leftmargin=*]
    \item \textbf{Popularity:} We rank the items based on their popularity and split the items into five groups, ensuring that each group contains an equal number of items.
    \item \textbf{Genre:} We categorize the items into different groups based on their respective genres. Each group consists of items that belong to the same class.
\end{itemize}

The popularity and the genre of an item differ in semantic aspects.
Specifically, the popularity of an item is semantic independent from the title of the item utilized as input for LLMs.
On the contrary, it is important to note that the genre of an item is intrinsically linked to its title. 
% Therefore, we conduct experiments on these two perspectives could help us probe the item-side fairness elaborately.
Therefore, by conducting experiments that consider both the popularity and genre perspectives, we can thoroughly probe the item-side fairness of LLMs for recommendations.

\subsubsection{Compared Method}
To demonstrate the item-side fairness of the LLMs for recommendations, and compare differences between conventional sequential recommendation methods and using LLMs for RS, we compare two methods respectively:
\begin{itemize}[leftmargin=*]
    \item \textbf{SASRec \cite{SASRec}:} This approach utilizes a self-attention mechanism, employing a left-to-right attention mechanism to acquire knowledge of sequential patterns and make predictions regarding the subsequent item. The SASRec is one of the representative works in conventional sequential recommendation methods.
    \item \textbf{BIGRec \cite{bigrec}:} The elaborate introduction can be seen in Section~\ref{sec:bigrec}. The BIGRec model stands as a notable example of leveraging LLMs for recommendations.
\end{itemize}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\caption{The item-side fairness of different methods for groups split by popularity.}
\label{tab:popularity_result}
\begin{tabular}{clllllllllll}
\hline
Dataset  & Model  & MGB@1           & MGB@3           & MGB@5           & MGB@10          & MGB@20          & DGB@1           & DGB@3           & DGB@5           & DGB@10          & DGB@20          \\ \hline
\multirow{2}{*}{MovieLens1M} & SASRec & \textbf{0.0238} & \textbf{0.0267} & \textbf{0.0279} & 0.0287          & 0.0279          & \textbf{0.0846} & \textbf{0.0925} & 0.0959          & 0.0976          & 0.0936          \\
                             & BIGRec & 0.1044          & 0.0447          & 0.0285          & \textbf{0.0178} & \textbf{0.0128} & 0.3917          & 0.1576          & \textbf{0.0956} & \textbf{0.0490} & \textbf{0.0383} \\ \hline
\multirow{2}{*}{Steam}       & SASRec & \textbf{0.0173} & \textbf{0.0168} & \textbf{0.0166} & \textbf{0.0162} & \textbf{0.0157} & \textbf{0.0647} & \textbf{0.0540} & \textbf{0.0485} & \textbf{0.0411} & \textbf{0.0445} \\
                             & BIGRec & 0.0411          & 0.0380          & 0.0590          & 0.0736          & 0.0900          & 0.1586          & 0.1374          & 0.1987          & 0.2460          & 0.3050          \\ \hline
\end{tabular}
\end{table*}

\subsection{Performance of Item-side Fairness Comparison}
In order to provide a more comprehensive response to \textbf{RQ2}, we have subdivided this question into two distinct aspects: Are LLMs for recommendations more fair for different groups split by popularity or genre of items?

\subsubsection{Diverse Popularity Groups}
\label{sec:diverse_pop_groups}
To answer the question \textbf{RQ2} of the popularity version, we evaluate the performance of mentioned methods, and comparison results are reported in Table~\ref{tab:popularity_result}.

Firstly, a clear distinction can be observed in Table~\ref{tab:popularity_result}, where it becomes evident that the BIGRec model performs inferiorly to SASRec in terms of $MGB$ until the top 5, and $DGB$ until the top 3 on the MovieLens1M dataset. 
Furthermore, the BIGRec model exhibits worse performance across all metrics on the Steam dataset. 

% Secondly, as shown in Table~\ref{tab:popularity_result}, it is worth noting that the SASRec and BIGRec models exhibit distinct patterns. 
% On MovieLens1M, the $MGB$ and $DGB$ from the top 1 to 20 of SASRec are nearly identical. 
% However, the metrics of BIGRec continue to decline with the increase of top $k$.
% Nevertheless, when examining the metrics of BIGRec: they consistently decrease as the value of top $k$ increases.
% On the Steam dataset, the SASRec still gets steady performance.
% But BigRec shows the opposite trend to the result on the MovieLens1M dataset.

Secondly, as shown in Table~\ref{tab:popularity_result}, it is worth noting that the SASRec and BIGRec models exhibit distinct patterns.
The SASRec exhibits steady performance on not only MovieLens1M but also Steam.
However, the BIGRec shows the opposite trend on two datasets.
On the MovieLens1M dataset, it is observed that the metrics of BIGRec exhibit a consistent decrease as the value of top $k$ increases. 
And the evaluation metrics of the BIGRec algorithm exhibit an initial decline followed by an upward trend as the value of top $k$ increases on the Steam dataset.

% \begin{figure}[!]
% \centerline{\includegraphics[width=0.4\textwidth]
% {}
% \caption{The result of meta-IRM with different number of samples and LightMIRM where $S$ denotes the number of samples.}
% % \vspace{-10pt}
% \label{fig:meta-IRM_complete}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{BIGRec_pop.pdf}
    \caption{Caption}
    \label{fig:proportion_of_pop}
\end{figure}

We further plot the proportion of recommendations of different groups on two datasets, to explore the reasons for this discrepancy. 
As depicted in Figure~\ref{fig:proportion_of_pop}, not only MovieLens1M but also Steam, the top 1 recommendation, which closely aligns with the base large language model's output, exhibits a notable degree of unfairness. 
Specifically, the proportions of groups 0 to 3 are observed to be lower than those observed in historical sequences.
And the proportion of group 4 in the top 1 recommendation exceeds its historical ratio.
This phenomenon means that the output of the base model is heavily influenced by popularity.





\subsubsection{Diverse Genre Groups}

\begin{table*}
\caption{The item-side fairness of different methods for groups split by genre}
\label{tab:genre_result}
\begin{tabular}{clllllllllll}
\hline
Dataset  & Model  & MGB@1           & MGB@3           & MGB@5           & MGB@10          & MGB@20          & DGB@1           & DGB@3           & DGB@5           & DGB@10          & DGB@20          \\ \hline
\multirow{2}{*}{MovieLens1M} & SASRec & \textbf{0.0048} & \textbf{0.0040} & \textbf{0.0037} & \textbf{0.0031} & \textbf{0.0025} & \textbf{0.0224} & \textbf{0.0207} & \textbf{0.0194} & \textbf{0.0172} & \textbf{0.0152} \\
                             & BIGRec & 0.0068          & 0.0076          & 0.0072          & 0.0065          & 0.0060          & 0.0374          & 0.0477          & 0.0418          & 0.0382          & 0.0383          \\ \hline
\multirow{2}{*}{Steam}       & SASRec & \textbf{0.0122} & \textbf{0.0114} & \textbf{0.0105} & 0.0092          & \textbf{0.0075} & \textbf{0.0477} & \textbf{0.0447} & \textbf{0.0452} & \textbf{0.0442} & 0.0403          \\
                             & BIGRec & 0.0158          & 0.0122          & 0.0106          & \textbf{0.0082} & 0.0081          & 0.0487          & 0.0532          & 0.0496          & 0.0443          & \textbf{0.0341} \\ \hline
\end{tabular}
\end{table*}


% To answer the question \textbf{RQ2} of the genre version, the comparison results are reported in Table~\ref{tab:genre_result}.

% According to the analysis presented in Table~\ref{tab:genre_result}, it can be observed that the BIGRec model achieves inferior performance compared to the SASRec model on almost all metrics. 

%
% Firstly, we observe the $MGB$ of the SASRec.

To answer the question \textbf{RQ2} of the genre version, we evaluate the fairness of SASRec and BIGRec for different genre groups, and the comparison results are reported in Table~\ref{tab:genre_result}.
The main observations are as follows:

\begin{itemize}[leftmargin=*]
    \item The SASRec model achieves superior performance compared to the BIGRec model on almost all metrics.
    Firstly, on the MovieLens1m dataset, both models have achieved relatively stable performance. 
    However, on the $DGB@3$ metric, BIGRec obtained poor results.
    On the Steam dataset, the evaluation metrics of both models decrease as the top $k$ increases. 
    Meanwhile, BIGRec shows a more significant decline in metrics.
    Hence, the fairness of the BIGRec begins to surpass the SASRec on high top $k$ recommendations.

    \item We will shift our focus to the evaluation metric of top1, as it better represents the fairness of the large language model itself. 
    We find that BIGRec performs worse on these metrics, especially on the DGB@1 metric, even surpassing SASRec 0.015 (\ie as much as 62.5\%).
    This implies that the large language model exhibits inferior fairness across different genre groups compared to SASRec.
    
    \item We further observe the difference between $MGB$ and $DGB$ of BIGRec. 
    The $MGB$ of BIGRec declines as the value of the top $k$ increases.
    For the $DGB$ metric, BIGRec reaches its peak when considering the top 3 recommendations.
    This implies that the second step for BIGRec could enhance the overall fairness of the model across various genre groups. 
    However, it may lead to more pronounced biases in certain specific categories.
    Consequently, using item title embeddings to align the recommendation output with the actual item space may potentially introduce fairness concerns pertaining to some specific genre groups.
\end{itemize}

\subsection{}
To answer \textbf{RQ3}, we perform a detailed comparison between semantic independence and semantic correlation scenarios. 
We have explored the impact of semantics on item-side fairness at different stages of using the large model for recommendation.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{BIGRec_genre.pdf}
    \caption{The group bias of different genre groups, where the \textit{HP} denotes the percentage of groups in historical interactions. The horizontal axis represents distinct genre groups, whose proportions in historical interactions increase from left to right.}
    \label{fig:genre_top1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{BIGRec_abalation.pdf}
    \caption{The proportion of genre groups in top 1 recommendation, where the \textit{HP} denote the percentage of groups in historical interactions and the \textit{RP} denote the proportion of genre groups in recommendation sequences. The horizontal axis represents distinct genre groups(\ie Documentary, Crime, Romance, Action, and Comedy), whose proportions in historical interactions increase from left to right.}
    \label{fig:genre_delete}
\end{figure}

Firstly, we probe the distinctions between two scenarios in the first step of BIGRec (\ie from language space to recommendation space).
Because the outputs in recommendation space may not exist in the real world, we utilize the top 1 recommendations instead.
In the semantic independence scenario, we have discovered that the large language model exhibits a preference for groups with higher popularity.
However, in the semantic scenario, the phenomenon is poised to become even more complex.
As shown in Figure~\ref{fig:genre_top1}, we split the images into two segments based on their proportions in historical interactions.
We find that more groups achieve negative group bias in the lower proportion segment(\aka MovieLens1M is 88\% and Steam is 66\%).
On the contrary, more groups obtain positive group bias in higher proportion segments (\aka MovieLens1M is 66\% and Steam is 60\%).
This suggests that large language models prefer groups with higher proportions.

To explore further factors that influence fairness across various genre groups, we propose additional experiments to uncover these factors. 
We select five genres in MovieLens1M and delete them in the training set.
And then, we verify the performance of large language model on these genre groups.
As shown in Figure~\ref{fig:genre_delete}, although we delete all items of these genre groups respectively, the large language model still recommends items in these groups.
This suggests that the large language model for recommendation is influenced by the previous corpus.
Specifically, we find that the \textit{Crime} and \textit{Romance} have comparable proportions in the recommendation sequences, but there is a significant disparity in historical interactions.
This implicit that the previous corpus could also result in an inherent injustice for various genre groups.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{BIGRec_special_genre.pdf}
    \caption{}
    \label{fig:special_genre}
\end{figure}

Secondly, we probe the distinctions in the second step of BIGRec.
In this step, the BIGRec bridges the outputs of large language model and item titles by embedding of them, grounding the outputs from recommendation space to actual item space.
As illustrated in Section~\ref{sec:diverse_pop_groups}, the popularity is independent of item titles.
Hence, in the semantic independent scenario, this step could mitigate the impact of popularity.
However, in the semantic correlation scenario, the genres and item titles are intricately intertwined.
As shown in Figure~\ref{fig:special_genre}, we find that the influence of the second step for various genre groups has three patterns.
Due to the non-uniformity of the embedding space, this step serves to mitigate the inherent unfairness present in certain genres. 
However, it is important to note that this process may introduce new fairness concerns for other genres or maintain the status.
This indicates that the impact of the second step of the approach on fairness across different genre groups will vary depending on the distribution of these groups in the embedding space.

\subsection{Summary}
The item-side fairness issues of LLMs for recommendations can be summarized in the following five categories. 
From semantics-independent perspective:
\begin{itemize}[leftmargin=*]
    \item Due to the imbalance of various groups, the large language model for recommendations discriminates against minorities.
    \item In the step of grounding of outputs from recommendation space to actual item space, the impact of imbalance could be mitigated. However, the overcorrection could occur in highly unbalanced data sets, which leads to injustice to majorities.
\end{itemize}

From semantics-dependent perspective:
\begin{itemize}[leftmargin=*]
    \item Similar to semantics-dependent perspective, the large language model for recommendations discriminates against minorities, which is split by the semantics-dependent criterion.
    \item The previous corpus for training large language models could also cause the model to be unfair to certain genre groups.
    \item Due to the item titles in various genre groups are not uniform in the embedding space, grounding outputs from recommendation space to actual item space could lead to injustice to certain genre groups.
\end{itemize}



